Stochastic vaccination game among influencers, leader and public

Celebrities can significantly influence the public towards any desired outcome. In a bid to tackle an infectious disease, a leader (government) exploits such influence towards motivating a fraction of public to get vaccinated, sufficient enough to ensure eradication. The leader also aims to minimize the vaccinated fraction of public (that ensures eradication) and use minimal incentives to motivate the influencers; it also controls vaccine-supply-rates. Towards this, we consider a three-layered Stackelberg game, with the leader at the top. A set of influencers at the middle layer are involved in a stochastic vaccination game driven by incentives. The public at the bottom layer is involved in an evolutionary game with respect to vaccine responses. We prove the disease can always be eradicated once the public is sufficiently sensitive towards the vaccination choices of the influencers -- with a minimal fraction of public vaccinated. This minimal fraction depends only on the disease characteristics and not on other aspects. Interestingly, there are many configurations to achieve eradication, each configuration is specified by a dynamic vaccine-supply-rate and a number -- this number represents the count of the influencers that needs to be vaccinated to achieve the desired influence. Incentive schemes are optimal when this number equals all or just one; the former curbs free-riding among influencers while the latter minimizes the dependency on influencers.

==> extra.tex <==
\subsection{Trying for $\nu_b$}



2) Given a base vaccination rate, the minimum possible vaccine rate at ESS 
$${\underline \nu}_k := \min_{(\nu_b, \nu_k): h_i(k) < 0,  h_v(k) < 0 } \{  \nu_b + \psi^*_e (\nu_k, \nu_b) \nu_k \}$$ 
which ensures CE (see ...),  decreases with increase in $k$  for $k  \ge {\bar k} (\nu_b)$.  


3) One can decrease the base vaccination rate and may improve CE possibilities  for a particular $k$ 


Thus in all, when $\delta $
is sufficiently small, it is optimal for leader to devise incentive scheme $g$ such that all influencers are vaccinated at the end of $T$ days.  This is optimal for both vaccinate rate supply and the expected cost towards incentives. Now design the minimum possible vaccine supply  rate   at ESS, for $k = M$ which will give the optimal $\nu^*.$


We saw that $k = M$ may not be the best when $\delta $ is big and variance is small or zero (perfect info). 
However even in this case, when the vaccine supply rate is of a bigger importance it would beneficial to choose an incentive scheme that ensures $k=M$. 
{\color{red} Observe here that all vaccine supply rates  beyond ${\underline \nu}_k$ ensure CE, however the smaller rates (of course more than or equal to ${\underline \nu}_k$) achieve the same with smaller fraction of public $\psi_k^*$ getting vaccinated.  

 }
For any feasible $\kappa$, there exists  a $\upsi$ and $\onu$ such that 
$$
h_i (k, \nu_b ) < 0 \mbox{ and }  h_v (k, \ps{e})  < 0 \mbox{ if }  \nu_b < \onu \mbox{ and }  \ps{e} (\nu_b, \nu) > \upsi. 
$$
 

Define, $V_k (\nu_b, \nu):= \nu_b + \psi^*_e (\nu_b, \nu) \nu$.
The aim is to find $(\nu_b, \nu)$ that solves the following
\begin{eqnarray}
    \inf_{(\nu_b, \nu) }  V_k (\nu_b, \nu) 
    \mbox{ s.t. } \ \   \ps{e} (\nu_b, \nu) > \upsi, \ \ \nu_b < \onu , \mbox{ and, }
    \nu_k > b \rho -\frac{\nu_b \rho}{\rho -1}.
    \label{Eqn_prob1}
\end{eqnarray}
It is easy to verify using the partial derivatives that      $\ps{e}$ (provided in Table \ref{table_ess_candidate}) and hence  $V_k$ are both strictly increasing with   $\nu_b$ as well as $\nu$. 
For every $\nu_b$ there exist a $\nu = \nuk(\nu_b) $ such that 
$\ps{e} (\nu_b, \nuk (\nu) ) = \upsi+\cst$, 
%and $\nuk (\nu) \ge b \rho - \nicefrac{\nu_b \rho}{\rho-1} + \cst$ (with equality in at least one of them),
where $\cst >0$ is a small constant.
Further by Lemma \ref{} of Appendix $L(\nu_b) :=  \nuk(\nu_b) - b \rho -\nicefrac{\nu_b \rho}{\rho -1}$ is increasing in $\nu_b$ and hence by feasibility  the problem \eqref{Eqn_prob1}
  is almost equivalent to (equivalence becomes better as $\delta \to 0$)
\begin{eqnarray*}
    \inf_{\nu_b }  V_k (\nu_b, \nuk(\nu_b)) 
    \mbox{ s.t. } \  \ \ \nu_b < \onu , \mbox{ and, }
    \nuk(\nu_b) > b \rho -\frac{\nu_b \rho}{\rho -1}.
\end{eqnarray*}
Clearly $V_k (\nu_b) := V_k (\nu_b, \nuk(\nu_b)) $ is monotone increasing function of $\nu_b$. 
The aim is to prove the existence of $\unu$ such that 
$$
\ps{e} (\nu_b, \nu) > \upsi,   \mbox{ and, }
    \nuk(\nu_b) > b \rho -\frac{\nu_b \rho}{\rho -1 }  \iff \nu_b >  \unu,
    $$
    which implies the ($\delta$) optimizer is $\unu.$ 



\begin{table}[h]

    \centering
    \begin{tabular}{|c||c|c|c||c||c|c|}
 
    \hline 
 $\baz$  & F1            & $\hat{p}_1$   &  cost  & F-2 & $g^*$ & cost* \\ 
         &  $\hat{g}_1$  &  &   &$\hat{g}_2$  & exact &  exact\\   \hline
 28      &  8.7      & 0.999   & 243.573     & 8.700    & 8.702    &  242.892\\ \hline 
 27      &  13.324   & 0.997   & 372.004     & 13.319   & 13.324   &  371.993\\ \hline  
 26      &  13.541   & 0.990   & 375.230     & 13.535   & 13.541   &  375.232 \\ \hline 
 25      &  13.599   & 0.978   & 372.491     & 13.590   & 13.599   &  372.519  \\ \hline      
 24      &  13.623   & 0.964   & 367.692     & 13.615   & &  \\ \hline 
 23      &  13.637   & 0.947   & 361.654     & 13.628   & & \\ \hline 
 22      &  13.646   & 0.928   & 354.701     & 13.637   & & \\ \hline
 21      &  13.652   & 0.908   & 347.004     & 13.643   & &  \\     \hline 
 20      &  13.656   & 0.886   & 338.670     & 13.647   & 13.656   &  338.583 \\ \hline
 19      &  13.660   & 0.862   & 329.767     & 13.651   & & \\ \hline
 18      &  13.663   & 0.837   & 320.345     & 13.654   & &  \\ \hline
 17      &  13.665   & 0.811   & 310.437     & 13.656   & &  \\ \hline
 16      &  13.667   & 0.784   & 300.066     & 13.658   & & \\ \hline
 15      &  13.668   & 0.756   & 289.245     & 13.660   &   13.668   &  289.259 \\ \hline
 14      &  13.670   & 0.726   & 277.982     & 13.662   & & \\ \hline
 13      &  13.671   & 0.696   & 266.276     & 13.664   & 13.6965 & 287.419\\ \hline
 12      &  13.672   & 0.664   & 254.123     & 13.665   &   13.672   &  254.214 \\ \hline
 11      &  13.673   & 0.631   & 241.507     & 13.667   & 13.674 & 241.823 \\ \hline
 10      &  13.674   & 0.597   & 228.409     & 13.668   &   13.645   &  228.527\\ \hline
 9       &  13.675   & 0.561   & 214.795     & 13.670   & & \\ \hline
 8       &  13.676   & 0.524   & 200.622     & 13.671   & & \\ \hline
 7       &  13.677   & 0.485   & 185.828     & 13.672   & & \\ \hline
 6       &  13.678   & 0.445   & 170.321     & 13.674   & & \\ \hline
 5       &  13.678   & 0.402   & 153.970     & 13.675   & 13.6785   &  154.112\\ \hline
 4       &  13.679   & 0.357   & 136.566     & 13.677   & 13.679   &  136.570 \\ \hline
 3       &  13.680   & 0.307   & 117.753     & 13.678   & 13.680   &  117.912 \\ \hline
 2       &  13.681   & 0.253   & 96.815      & 13.680    &    13.681   &  96.901 \\ \hline
 1       &  13.682   & 0.187   & 71.775      & 13.682    &  13.682   &  71.948\\ \hline
      
    \end{tabular}
    \caption{{\bf small variance, small delta, approximations and exact values}\\$\nu_z (z) = \nu + z \nu_z$, $\delta = 0.003$, $M=28$, $\lambda = 38$, $r=2$, $b=6$, $\gamma =0.6$ (discount factor for $\CI$), $T=10$, $M_{max}=50$, $c=1$, $\mvs=14$, $\hat{\sigma}=0.002$ (Normal), $c_{v1}=0.2$, $c_{v2}=0.05$, $\bar{c}_{v2}=0.5$, $c_{i}=2$, $c_f(\zt)=\zt$, $C_v=1$, $\CI=\frac{c_{i}}{1-\gamma}$.} 
    \label{tab:my_label}
    
\end{table}

\begin{table}[h]

    \centering
    \begin{tabular}{|c||c|c|c||c||c|c|}
 
    \hline 
 $\baz$  & F1     & $\hat{p}_1$   &  cost  & F-2 & $g^*$ & cost* \\ 
         &  $\hat{g}_1$  &  &   &$\hat{g}_2$  &  &  \\   \hline

 28      &  8.700   & 0.992   & 241.666     & 8.700   & 8.70046 & 193.104 \\ \hline
 27      &  10.925   & 0.970   & 296.871     & 10.595   & & \\ \hline
 26      &  11.477   & 0.945   & 303.588     & 10.979   & & \\ \hline
 25      &  11.741   & 0.917   & 301.408     & 11.145   &11.7410   &  301.425 \\ \hline
 24      &  11.900   & 0.888   & 295.790     & 11.245   & & \\ \hline
 23      &  12.010   & 0.858   & 288.382     & 11.319   & & \\ \hline
 22      &  12.091   & 0.827   & 279.872     & 11.380   & & \\ \hline
 21      &  12.154   & 0.795   & 270.607     & 11.436   & & \\ \hline
 20      &  12.206   & 0.763   & 260.783     & 11.489   &  12.2060   &  260.782 \\ \hline
 19      &  12.249   & 0.730   & 250.523     & 11.540   & & \\ \hline
 18      &  12.286   & 0.697   & 239.904     & 11.590   & & \\ \hline
 17      &  12.319   & 0.664   & 228.981     & 11.640   & & \\ \hline
 16      &  12.348   & 0.630   & 217.791     & 11.690   & & \\ \hline
 15      &  12.373   & 0.596   & 206.360     & 11.741   & 12.3760   &  206.455\\ \hline
 14      &  12.397   & 0.561   & 194.708     & 11.793   & & \\ \hline
 13      &  12.419   & 0.526   & 182.846     & 11.845   & & \\ \hline
 12      &  12.439   & 0.490   & 170.782     & 11.898   & & \\ \hline
 11      &  12.458   & 0.454   & 158.519     & 11.953   & & \\ \hline
 10      &  12.476   & 0.418   & 146.057     & 12.008   &     12.4760   &  146.051 \\ \hline
 9      &  12.494   & 0.381   & 133.390     & 12.065   & & \\ \hline
 8      &  12.510   & 0.344   & 120.506     & 12.124   & & \\ \hline
 7      &  12.527   & 0.306   & 107.389     & 12.185   & & \\ \hline
 6      &  12.543   & 0.268   & 94.011     & 12.248   & & \\ \hline
 5      &  12.560   & 0.228   & 80.329     & 12.314   &   12.5600   &  80.334    \\ \hline
 4      &  12.577   & 0.188   & 66.276     & 12.384   & & \\ \hline
 3      &  12.595   & 0.147   & 51.732     & 12.459   & & \\ \hline
 2      &  12.615   & 0.103   & 36.452     & 12.542   & & \\ \hline
 1      &  12.641   & 0.056   & 19.771     & 12.641   &  12.6720   &  20.190 \\ \hline      
    \end{tabular}
    \caption{{\bf small variance, big delta, approximations and exact values}\\$\nu_z (z) = \nu + z \nu_z$, $\delta = 0.2$, $M=28$, $\lambda = 38$, $r=2$, $b=6$, $\gamma =0.6$ (discount factor for $\CI$), $T=10$, $M_{max}=50$, $c=1$, $\mvs=14$, $\hat{\sigma}=0.002$ (Normal), $c_{v1}=0.2$, $c_{v2}=0.05$, $\bar{c}_{v2}=0.5$, $c_{i}=2$, $c_f(\zt)=\zt$, $C_v=1$, $\CI=\frac{c_{i}}{1-\gamma}$.} 
    \label{tab:my_label}
    
\end{table}



{\begin{table}[h]

    \centering
    \begin{tabular}{|l|c||c|c||c|c||c|c|c|c|}
 
    \hline 
    $\nu$, $\nu_z$     &  $\baz$  & $g^*$     & overall   & $g^*$  & overall  & $g^*$  & overall  \\ 
    &    & $\delta = 0.2$  & $\delta = 0.2$ & $\delta = 0.3, 0.1, 0.01, 0.001$ &  $\delta = 0.3, 0.1, 0.01, 0.001$ & $\delta = 0.05$  &   $\delta = 0.05$
    \\
    \hline
      $(1.1, 1)$       &  28      &  9.89     & 220.65  & 9.44, 10.51, 11.96, 12.99 & 185, 264.62, 331.36, 363.54 & 11.04   & 293.9 \\ \hline 
      $(0.001, 1.05)$  &  28      &  9.876    & 220.47  &  &    & 11.03    & 293.54 \\ \hline       
      $(1, 1.01)$      &  27      &  11.48    &  305.23 &  &  & 13.07   & 362.30 \\ \hline 
      $(1.1, 1.05)$    &  26      &  11.90    &  312.90 &  &  & 13.52   & 371.44 \\ \hline 
      $(1.1, 1.1)$     &  25      &  12.12    &  312.24 &  &  & 13.76   & 374.36 \\ \hline       
      $(1.1, 1.15)$    &  24      &  12.26    &  308.70 &  &  & 13.88   & 372.27 \\ 
      \hline       
      $(5.1, 1.1)$     &  21      &  12.45    & 289.50  &  &  & 14.12   & 369.32 \\     \hline     
      $(1.1, 2.1)$     &  13      &  12.69    & 224.44  &  &  & 14.34   & 343.40 \\ 
      \hline     
      $(1.1, 2.8)$     &  10      &  12.78    &  201.37 &  &  & 14.30   & 325.50 \\ 
      \hline      
      $(5.1, 5.1)$     &   5      &  12.87    & 159.80  &  &  & 14.34    & 306.80 \\ 
      \hline 
      $(10.1, 10.1)$   &   2      &  12.92   & 129.50   &  &  & 14.46    & 301.3  \\ \hline  
      $(15.1, 17.1)$   &   1      &  12.93   & 121.29   &12.247, 13.76, 15.65, 16.90  &67.17, 213.23, 405.02, 468.23  & 14.49    & 301.31 \\ \hline   
      
    \end{tabular}
    \caption{$\nu_z (z) = \nu + z \nu_z$, $\delta = 0.2$, $M=28$, $\lambda = 38$, $r=2$, $b=6$, $\gamma =0.6$ (discount factor for $\CI$), $T=10$, $M_{max}=50$, $c=1$, $\mvs=14$, $\hat{\sigma}=5$ (Normal), $c_{v1}=0.2$, $c_{v2}=0.05$, $\bar{c}_{v2}=0.5$, $c_{i}=2$, $c_f(\zt)=\zt$, $C_v=1$, $\CI=\frac{c_{i}}{1-\gamma}$.} 
    \label{tab:my_label}
    
\end{table}
}


\begin{table}[h]

    \centering
    \begin{tabular}{|c||c|c||l|l||}
 
    \hline 
 $\baz$  & $\delta = 0.003$    &  cost  & $\delta = 0.2$  & cost  \\ 
         &  $g$                &        & $g$              &    \\   \hline
28 & 10.2630   &  286.555  & 9.17   & 204.536 \\ \hline
27 & 13.75     & 384.388   & 11.01  & 299.247 \\ \hline
25 & 14.22     & 395.943   & 11.79  & 303.0988\\ \hline
20 & 14.4      & 396.631   & 12.235 & 262.818 \\ \hline
15 & 14.462    & 394.101   & 12.4   & 209.896 \\ \hline
12 & 14.477    & 391.720   & 12.46  & 175.460 \\ \hline
10 & 14.492    & 390.282   & 12.5   & 152.057 \\ \hline
5  & 14.524    & 386.310   & 12.6   & 89.716 \\ \hline
2  & 14.54     &  384.284  & 12.6319& 47.276 \\ \hline
1  & 14.55     & 383.67    & 12.67  & 33.0518 \\ \hline

    \end{tabular}
    \caption{{\bf big variance, small 
 and big delta, exact values}\\$\nu_z (z) = \nu + z \nu_z$, $\delta = 0.003$ and 0.2, $M=28$, $\lambda = 38$, $r=2$, $b=6$, $\gamma175.460 =0.6$ (discount factor for $\CI$), $T=10$, $M_{max}=50$, $c=1$, $\mvs=14$, $\hat{\sigma}=2$ (Normal), $c_{v1}=0.2$, $c_{v2}=0.05$, $\bar{c}_{v2}=0.5$, $c_{i}=2$, $c_f(\zt)=\zt$, $C_v=1$, $\CI=\frac{c_{i}}{1-\gamma}$.} 
    \label{tab:my_label}
    
\end{table}

{
\begin{table}[h]

    \centering
    \begin{tabular}{|l|c||c|c||c|c||c|c|c|c|}
 
    \hline 
    $\nu$, $\nu_z$     &  $\baz$  & $g^*$     & $p^*$   &  approx $\hat{g}$  & approx $\hat{p}$   & variance  & variance \\ 
            &    &  &  & $\hat{g}$  &$\hat{p}$   &  0.2  $g^*$     & 0.2 $p^*$   \\ 

      \hline
      $(1.1, 1)$       &  28      &  8.7   & 0.999990  & 8.7 &  & 11.04   & 293.9 \\ \hline 
      $(0.001, 1.05)$  &  28      &  9.876    & 220.47  &  &    & 11.03    & 293.54 \\ \hline       
      $(1, 1.01)$      &  27      &  11.48    &  305.23 &  &  & 13.07   & 362.30 \\ \hline 
      $(1.1, 1.05)$    &  26      &  11.90    &  312.90 &  &  & 13.52   & 371.44 \\ \hline 
      $(1.1, 1.1)$     &  25      &  12.12    &  312.24 &  &  & 13.76   & 374.36 \\ \hline       
      $(1.1, 1.15)$    &  24      &  12.26    &  308.70 &  &  & 13.88   & 372.27 \\ 
      \hline       
      $(5.1, 1.1)$     &  21      &  12.45    & 289.50  &  &  & 14.12   & 369.32 \\     \hline     
      $(1.1, 2.1)$     &  13      &  12.69    & 224.44  &  &  & 14.34   & 343.40 \\ 
      \hline     
      $(1.1, 2.8)$     &  10      &  12.78    &  201.37 &  &  & 14.30   & 325.50 \\ 
      \hline      
      $(5.1, 5.1)$     &   5      &  12.87    & 159.80  &  &  & 14.34    & 306.80 \\ 
      \hline 
      $(10.1, 10.1)$   &   2      &  12.92   & 129.50   &  &  & 14.46    & 301.3  \\ \hline  
      $(15.1, 17.1)$   &   1      &  12.93   & 121.29   &  & & 14.49    & 301.31 \\ \hline   
      
    \end{tabular}
    \caption{{\bf small variance, small delta, approximations and exact values}\\$\nu_z (z) = \nu + z \nu_z$, $\delta = 0.2$, $M=28$, $\lambda = 38$, $r=2$, $b=6$, $\gamma =0.6$ (discount factor for $\CI$), $T=10$, $M_{max}=50$, $c=1$, $\mvs=14$, $\hat{\sigma}=0.2$ (Normal), $c_{v1}=0.2$, $c_{v2}=0.05$, $\bar{c}_{v2}=0.5$, $c_{i}=2$, $c_f(\zt)=\zt$, $C_v=1$, $\CI=\frac{c_{i}}{1-\gamma}$.} 
    \label{tab:my_label}
    
\end{table}

\begin{table}[h]

    \centering
    \begin{tabular}{|l|c||c|c||c|c||c|c|c|c||c|c|c|c|}
 
    \hline 
    $\nu$, $\nu_z$     &  $\baz$  & $g^*$           & overall         &  $g^*$           & overall          &  $g^*$           & overall  \\ 
                       &          & $\delta = 0.2$  & $\delta = 0.2$  & $\delta = 0.05$  &   $\delta = 0.05$  & $\delta = 0.01$  &   $\delta = 0.01$
    \\
    \hline
      $(1.1, 1)$       &  28      &  9.89     & 220.65     & 11.04   & 293.9  & &\\ \hline 
      $(0.001, 1.05)$  &  28      &  9.876    & 220.47     & 11.03   & 293.54   & & \\ \hline       
      $(1, 1.01)$      &  27      &  11.48    &  305.23    & 13.07   & 362.30   & &\\ \hline 
      $(1.1, 1.05)$    &  26      &  11.90    &  312.90    & 13.52   & 371.44   & &\\ \hline 
      $(1.1, 1.1)$     &  25      &  12.12    &  312.24    & 13.76   & 374.36   & &\\ \hline       
      $(1.1, 1.15)$    &  24      &  12.26    &  308.70    & 13.88   & 372.27   & &\\ 
      \hline       
      $(5.1, 1.1)$     &  21      &  12.45    & 289.50     & 14.12   & 369.32  & &\\     \hline     
      $(1.1, 2.1)$     &  13      &  12.69    & 224.44     & 14.34   & 343.40  & &\\ 
      \hline     
      $(1.1, 2.8)$     &  10      &  12.78    &  201.37    & 14.30   & 325.50  & &\\ 
      \hline      
      $(5.1, 5.1)$     &   5      &  12.87    & 159.80     & 14.34    & 306.80  & &\\ 
      \hline 
      $(10.1, 10.1)$   &   2      &  12.92   & 129.50      & 14.46    & 301.3  & & \\ \hline  
      $(15.1, 17.1)$   &   1      &  12.93   & 121.29      & 14.49    & 301.31 & & \\ \hline   
      
    \end{tabular}
    \caption{$\nu_z (z) = \nu + z \nu_z$, $\delta = 0.2$, $M=28$, $\lambda = 38$, $r=2$, $b=6$, $\gamma =0.6$ (discount factor for $\CI$), $T=10$, $M_{max}=50$, $c=1$, $\mvs=14$, $\hat{\sigma}=5$ (Normal), $c_{v1}=0.2$, $c_{v2}=0.05$, $\bar{c}_{v2}=0.5$, $c_{i}=2$, $c_f(\zt)=\zt$, $C_v=1$, $\CI=\frac{c_{i}}{1-\gamma}$.} 
    \label{tab:my_label}
    
\end{table}

}





We will now show below that $\baz=M$ is also  optimal from the perspective of vaccine supply cost. Our eventual conclusion regarding the joint optimal strategy for small enough value of $\delta$ is two fold: i)  compelling all the influencers to get vaccinated, i.e., achieving $Z_T =M$ a.s., by using incentive scheme $g^*_M$ and ii) using a VA strategy optimal for $\baz = M$ derived below.


Our goal now is to derive a VA strategy
that ensures CE and also minimizes the eventual rate of vaccination  at ESSS, i.e., $\nu_b + \nu_e \ps{e}(\bnu)$. 

We achieve this by having a different outlook towards the problem, 
we first we consider all possible $k$ that are achievable for some vaccine rate pair and then discuss the pairs that achieve minimum vaccination rate at equilibrium and still ensure CE. 



1) Given an instance of problem (including base vaccination rate), there exists a ${\baz} (\nu_b)<M$ such that  CE is not possible for all $k < {\baz}$. 

For the CE given  number of vaccinated influencers $\Zt = \zt$, one requires three conditions: i) $h_i(\zt)<0$, ii) $h_v(\zt)<0$ and iii) $\nu_e > b \rho  - \frac{\nu_b \rho}{\rho -1}$.


Given the base vaccination rate $\nu_b$,  the function $h_i(\cdot)$ in first condition equals,
$$ h_i (k)  = c_{v_1} + \left(1-\frac{\zt}{M}\right)\bar{c}_{v_2} - \frac{\lambda \bar{\theta}^*}{\lambda \bar{\theta}^*+\nu_b} c_{i} - c_f(\zt). $$
If $h_i(0)<0$, then set $\Bar{k}_1(\nu_b)=1$, however if  $h_i(0)>0$ then there exist some $0<k\le M$ such that $h_i(k)<0$, since $h_i(M)<0$ and $h_i(\cdot)$ is a strict monotone decreasing function. Let $\Bar{k}_1(\nu_b)$ be largest  $k$ such that $h_i(k)>0$, then from monotonicity of $h_i(\cdot)$,  $h_i(k')>0$ for all $k' \le \Bar{k}_1(\nu_b)$ .
Now, consider second condition,  for any given $k$, the smallest value $h_v(k)$ can take is (see \eqref{eqn_utility}),
$$h_v(k) =c_{v_1} + \left(1-\frac{\zt}{M}\right)\frac{c_{v_2}}{\ps{e}} - c_f(\zt) \ge c_{v_1} + \left(1-\frac{\zt}{M}\right)c_{v_2} - c_f(\zt):={\underline h}_v(k) .$$
If ${\underline h}_v(k) >0$ for some $k$, then from monotonicity,  ${\underline h}_v(k') >0$ for all $k'\le k$. Let  $\Bar{k}_2$ be largest  $k$ such that $h_v(k)>0$. Then $\Bar{k}(\nu_b) = \max\{\Bar{k}_1(\nu_b),\Bar{k}_2\} +1
$. Further, observe that one can achieve CE for every $k > \Bar{k}(\nu_b) $, since $\ps{e}$ can increase to 1 by increasing $\nu_k$ from Lemma \ref{} in appendix \ref{appendix_leaders_game}. By lemma \ref{}, there is a $\Bar{\nu}$ such that $h_v(k)<0$. 

Now, we discuss the minimum equilibrium (at ESSS) vaccination rate required to achieve  CE for a $k \ge \Bar{k}(\nu_b)$, once the basic vaccination rate is fixed. The extra vaccination rate (in addition to $\nu_b$) is given by:
\begin{eqnarray*}
    {\underline \nu}^*_k  := \inf_{\nu} & \ \ \psi^*_e (\nu) \nu,& \\
    \mbox{s.t.}&  h_v(k;\nu) &<0,
    \\
   &  \nu &> b \rho -\frac{\nu_b \rho}{\rho -1}.
\end{eqnarray*}By Lemma \ref{lem_variation_psi} of appendix \ref{appen_ode}, $\ps{e} (\nu)$ is increasing in $\nu$, $h_v(k;\cdot)$ is decreasing. Other constraint is obviously monotone in $\nu$. Let  $\nu_1 :=  b \rho -\frac{\nu_b \rho}{\rho -1}$, and $\nu_{(2,k)}$ satisfy $h_v(k;\nu_{(2,k})) =0$, which is unique by monotonicity.  Further,  by  monotonicity of the involved functions and the objective function, it is easy to verify that the infimum is ${\underline \nu}^*_k = \nu_b + \psi^*_e (\nu^*_k, \nu_b) \nu_k$ where $\nu_k = \max\{\nu_1,\nu_{(2,k}\} $. Further $h_v(\cdot;\nu)$ is  strictly decreasing  in $k$  when $\nu$ is fixed, and thus $h_v(k';\nu_{(2,k})) < h_v(k;\nu_{(2,k}))$ which implies  $\nu_{(2,k')} >\nu_{(2,k)}$  when $k'>k$. Finally, by
 monotonicity of $\ps{e}$, the infimum equilibrium vaccination rate required for CE is smaller for larger $k$, i.e.,
${\underline \nu}^*_{k'}<{\underline \nu}^*_{k}$. 


\rcmnt{
\begin{itemize}
    \item The fraction of people who have to be vaccinated to achieve CE for any $\zt$
    \item expenditure due to incentives 
    \item extra vaccination rate for esss
\end{itemize}


-- picture of $\ps{e}$ for the optimal $\nu_k$ for all $k$ }.
\newpage\section*{Not required material}
Now our aim is to prove the existence of vaccine-optimal strategy. Towards this, we define the following: 

{\small
\begin{eqnarray}\label{eqn_k_star}
k_1 &: =& \min \left\{k : c_{v_1} + \frac{c_{v_2}}{\nvdf}\left(1-\frac{k}{M}\right) - c_f(k)<0\right\},\nonumber\\
k_2 &: =& \min \left\{k : c_{v_1} + \bar{c}_{v_2}\left(1-\frac{k}{M} \right) - c_f(k)<c_i\right\}, \mbox{ and }\\
\bar{k}_2 &:=& \min \left\{k : c_{v_1} + \bar{c}_{v_2}\left(1-\frac{k}{M} \right) - c_f(k)< 0\right\}, \mbox{ and }
k^* := \max\{k_1, k_2\}. \nonumber
\end{eqnarray}}
\vcmnt{Towards part (ii), we need $\baz(\bnu)=M$ and $\bnu$ to be $\epsilon$-vaccine-optimal. From theorem \ref{thm_vaccine_optimal}, existence of such a strategy is equivalent to the case when $\Bar{k}_2=M$ and \eqref{eqn_iff_k_bar_eps} is true, which is precisely \eqref{eqn_inc_vac_optimal}. \eop}


%\input{psi_inf.tex}
\textbf{proof of $\baz(\bnu)=k^*$ }Further, to prove $\baz(\bnu^\epsilon) = k^*$, we need to prove that $h_i(k^*;\bnu^\epsilon)<0$, $h_v(k^*;\bnu^\epsilon)<0$  and either $h_i(k^*-1;\bnu^\epsilon)>0$ or $h_v(k^*-1;\bnu^\epsilon)>0$ (see theorem \ref{thm_eradication_es}). 
%
Now, by definition of $k^*$ in \eqref{eqn_k_star} and \eqref{eqn_h_func} $h_v(k^*;\bnu^\epsilon)<0$ since $\ps{e}(\bnu^\epsilon) > \nvdf$ by lemma \ref{lem_min_psi}. Further,  if required $\nu_b$ can be reduced sufficiently so that $h_i(k^*;\bnu^\epsilon)<0$.
Further,   either $k^*=k_1$ or $k^* = k_2$ of \eqref{eqn_k_star}. If $k^*=k_1$, then $h_v(k^*-1;\bnu)>0$ and if $k^*=k_2$, then $h_i(k^*-1;\bnu)>0$.
Hence part (i) is true.


Now consider the first term. From continuity of $p(g_{\sigma},\cdot)$ by  lemma \ref{lem_monotonicity_of_p},
for any $\epsilon_1>0$, there exists an $\epsilon_2$ such that $\mid p(g_{\sigma},c)-p(g_{\sigma},c^*)\mid < \epsilon_1$ if $\mid c- c^* \mid<\epsilon_2$. Thus,
%
$$A:=\{\omega: \mid C_{\sigma}(\omega)-c^*
\mid \le \epsilon_2\} \subset \{\omega: \mid p(g_{\sigma},C_{\sigma}(\omega))-p(g_{\sigma},c^*)
\mid \le \epsilon_2\}. $$
Now, 
\begin{eqnarray*}
    \mid  E[p(g_{\sigma},\Gmcs)] - p(g_{\sigma},\Gmcm) \mid &=& \mid  E[p(g_{\sigma},\Gmcs) - p(g_{\sigma},\Gmcm)] \mid,\\
    & \le & \epsilon_1 + P(\mid C_{\sigma}(\omega)-c^*
\mid > \epsilon_2)<\epsilon_3,
\end{eqnarray*} when $n\ge N$ since $C_{\sigma}\stackrel{L^1}{\to}c^*$ and hence $C_{\sigma}\stackrel{p}{\to}c^*$.

 For the second term, from part (iii) and since $p(\cdot,\Gmcm)$ is a continuous function,  $p(g_{\sigma},\Gmcm) \to p(g^*,\Gmcm)$, where $g^*$ is given by \eqref{eqn_perf_opt}. Further, from \eqref{eqn_outcome_vaccination}, observe that $ p(g^*,\Gmcm)$ satisfies,
\begin{eqnarray*}
    F_{M-1}(\baz-1;p(g^*,\Gmcm))& =& \frac{C_v - g^* +\Gmcs }{C_i}=F_{M-1}(\baz-1;p^*),
\end{eqnarray*}by substituting $g^*$ from \eqref{eqn_leader_opt}. Thus, $p(g^*,\Gmcm) = p^*$ and from \eqref{eqn_app_convg}, we have $E[p(g_{\sigma},\Gmcs)] \to p^*$. Hence $\Ui_k^*(\sigma^2) \to M g^* p^*= \Ui^*_k$ further using part (iii). 
\eop

Towards part (iii), say \eqref{eqn_inc_vac_optimal} holds. If $-\frac{c_{v_2}}{M\nvdf}<\frac{r+b}{r+2b}c_i- \frac{\bar{c}_{v_2}}{M}$, then  from \eqref{eqn_h_func}, $h_v(M-1)>0$. Otherwise choose $\bnu^\epsilon$ such that $\nu_b\le b \rho \nvdf$ and $\nu_e = b\rho - \frac{\nu_b}{\nvdf}+\tilde{\epsilon}$ as in lemma \ref{lem_min_psi}(iv), then $h_i(M-1)>0$ and $\ps(\bnu^\epsilon)<\nvdf+\epsilon$. Thus $\baz(\bnu^\epsilon)=M$ and then choose $g^\epsilon$ that solves \eqref{eqn_leader_opt_wait} with $\baz=M$. Then $(g^\epsilon,\bnu^\epsilon)$ is an incentive-optimal strategy. 
Now consider the converse. Say for a given $\epsilon>0$, $(g^{\epsilon},\bnu^{\epsilon})$ is a policy with $\bnu^\epsilon = (\nu_b^\epsilon,\nu_e^\epsilon)$ which is incentive optimal as well as vaccine optimal, i.e., $\ps{e}(\bnu^{\epsilon}) - \nvdf = \epsilon'<\epsilon$, and $\baz(\bnu^{\epsilon})=M$. Further, for incentive optimality, we have either,
%

\vspace{-3mm}
{\small
\begin{eqnarray}\label{eqn_both_opt2}
  c_{v_1} - c_f(M-1) &>&   -  \frac{c_{v_2}}{M(\nvdf+\epsilon')}, \hspace{1cm}\\
  c_{v_1} - c_f(M-1) &>&  \frac{\lambda \nvdf}{\lambda \nvdf + \nu_b^{\epsilon}} c_i -  \frac{\bar{c}_{v_2}}{M} = \frac{r+b}{r+2b +b (\frac{\nu_b^{\epsilon}}{b \rho \nvdf}-1)} c_i -  \frac{\bar{c}_{v_2}}{M}. \hspace{1cm}\label{eqn_both_opt1}
\end{eqnarray}}%
for $h_v(M-1;\bnu^{\epsilon})>0$ or for $h_i(M-1;\bnu^{\epsilon})>0$ respectively. If in the optimal policy $\bnu^{\epsilon}\le b\rho \nvdf$, then as $\epsilon \to 0$, we have \eqref{eqn_inc_vac_optimal}. However if $\nu_b^{\epsilon}>b\rho\theta^*$ in the optimal policy, then from the monotonicity of $\ps{e}(\bnu^{\epsilon})$ from lemma \ref{lem_min_psi}, as $\epsilon\to 0$, $\nu_b^\epsilon \to b \rho \theta^*$, and again we get \eqref{eqn_inc_vac_optimal}.\eop


\subsection*{Right hand partial derivative  of $\ps{e}(\bnu)$ at $\nu_e=0$:}

\vspace{-3mm}
{\small
\begin{eqnarray*}
\eval{\pdv{ \ps{e}(\bnu)}{\nu_e}}_{\nu_e=0} &=& \lim_{h\downarrow 0} \frac{ \ps{e}(\nu_b, h) -  \ps{e}(\nu_b,0)}{h},\\
&& \hspace{-2cm}= \lim_{h\downarrow 0}\frac{ \frac{-(b +\nu_b-h)+\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}}{2 h } - \frac{\nu_b}{b+\nu_b}}{h}, \ \mbox{ (apply L'Hopital) },\\
%2
&& \hspace{-3cm}= \lim_{h\downarrow 0}\frac{2h \left(1 + \frac{-2(b +\nu_b-h) + 4 \nu_b}{2\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}}\right)- 2[-(b +\nu_b-h)+\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}]}{4 h^2 } ,\\
%3
&& \hspace{-3cm}= \lim_{h\downarrow 0}\frac{h \left(1 + \frac{-b +\nu_b +h}{\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}}\right)+ (b +\nu_b-h)-\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}}{2h^2 } ,\ \mbox{ (apply L'Hopital) },\\
%L hopital
&& \hspace{-3cm}{=} \lim_{h\downarrow 0}\frac{\left(h \frac{(b +\nu_b-h)^2 + 4 h \nu_b- (-b +\nu_b +h)^2 }{((b +\nu_b-h)^2 + 4 h \nu_b)^{\frac{3}{2}}}+1 + \frac{-b +\nu_b +h}{\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}}\right)-  \left(1 + \frac{-b +\nu_b+h}{\sqrt{(b +\nu_b-h)^2 + 4 h \nu_b}}\right)}{4h } ,\\
%
&& \hspace{-3cm}=\lim_{h\downarrow 0}\frac{(b +\nu_b-h)^2 + 4 h \nu_b- (-b +\nu_b +h)^2 }{4((b +\nu_b-h)^2 + 4 h \nu_b)^{\frac{3}{2}}}  = \frac{(b +\nu_b)^2 - (-b +\nu_b )^2 }{4(b +\nu_b) )^{3}}>0.
\end{eqnarray*}}\eop


\subsection*{Both optimality}
\begin{cor}\label{cor_both_opt}
There exists a policy $(\bg,\bnu^\epsilon)$ which is incentive-optimal as well as $\epsilon$-vaccine-optimal if and only if,
\begin{equation}\label{eqn_inc_vac_optimal}
    c_{v_1} -c_f(M-1)   > \min\left\{-\frac{c_{v_2}}{M\nvdf},\  \  \frac{r+b}{r+2b}c_i - \frac{\bar{c}_{v_2} }{M}\right\}. 
\end{equation}
\end{cor}
\noindent\textbf{Proof of corollary \ref{cor_both_opt}:} Say \eqref{eqn_inc_vac_optimal} holds. If $-\frac{c_{v_2}}{M\nvdf}<\frac{r+b}{r+2b}c_i- \frac{\bar{c}_{v_2}}{M}$, then  from \eqref{eqn_h_func}, $h_v(M-1)>0$. Otherwise choose $\bnu^\epsilon$ such that $\nu_b\le b \rho \nvdf$ and $\nu_e = b\rho - \frac{\nu_b}{\nvdf}+$ as in lemma \ref{lem_min_psi}(iv), then $h_i(M-1)>0$ and $\ps{e}(\bnu^\epsilon)<\nvdf+\epsilon$. Thus $\baz(\bnu^\epsilon)=M$ and then choose $\bg$ that solves \eqref{eqn_leader_opt} with $\baz=M$. Then $(\bg,\bnu^\epsilon)$ is an incentive-optimal as well as $\epsilon$-vaccine-optimal strategy. 
Now consider the converse. Say for a given $\epsilon>0$, $(\bg,\bnu^{\epsilon})$ is a policy with $\bnu^\epsilon = (\nu_b^\epsilon,\nu_e^\epsilon)$ which is incentive optimal as well as vaccine optimal, i.e., $\ps{e}(\bnu^{\epsilon}) - \nvdf = \epsilon'<\epsilon$, and $\baz(\bnu^{\epsilon})=M$. Further, for incentive optimality, we have either,
%

\vspace{-3mm}
{\small
\begin{eqnarray}\label{eqn_both_opt2}
  c_{v_1} - c_f(M-1) &>&   -  \frac{c_{v_2}}{M(\nvdf+\epsilon')}, \hspace{1cm}\\
  c_{v_1} - c_f(M-1) &>&  \frac{\lambda \nvdf}{\lambda \nvdf + \nu_b^{\epsilon}} c_i -  \frac{\bar{c}_{v_2}}{M} = \frac{r+b}{r+2b +b (\frac{\nu_b^{\epsilon}}{b \rho \nvdf}-1)} c_i -  \frac{\bar{c}_{v_2}}{M}. \hspace{1cm}\label{eqn_both_opt1}
\end{eqnarray}}%
for $h_v(M-1;\bnu^{\epsilon})>0$ or for $h_i(M-1;\bnu^{\epsilon})>0$ respectively. If in the optimal policy $\bnu^{\epsilon}\le b\rho \nvdf$, then as $\epsilon \to 0$, we have \eqref{eqn_inc_vac_optimal}. However if $\nu_b^{\epsilon}>b\rho\theta^*$ in the optimal policy, then from the monotonicity of $\ps{e}(\bnu^{\epsilon})$ from lemma \ref{lem_min_psi}, as $\epsilon\to 0$, $\nu_b^\epsilon \to b \rho \theta^*$, and again we get \eqref{eqn_inc_vac_optimal}.\eop

\section{old abstract}

A leader, a set of influencers and general public form three layers of agents in our Stackelberg vaccination game, where the leader in the top layer aims to ensure complete eradication of an ongoing pandemic with required level of certainty. 
The aim of the leader is actually   three fold -- ensure complete eradication, have minimal  vaccinated fraction of public, and using optimal incentive scheme. The end result depends significantly on the level of sensitivity of the vaccine response of the public upon that of the influencers; more interestingly it is non-monotone in the sensitivity level. The free-riding behaviour of the public and that of the influencers are causes for it. An evolutionary stable equilibrium  at public level with almost all public vaccinated  is achieved by curbing the free-riding   behaviour of both the public and the influencers. 

If the aim is also to vaccinate optimal fraction of public, the 
If the public is significantly influenced by influencers, leader can provide minimal  incentives to  the influencers--the free-riding behaviour of the public is curbed.  When the public is public is least influenced, the leader can again provide minimal incentives -- at equilibrium the free-riding behaviour of the influencers is curbed. For intermediate levels of influence the leader spends significantly on incentives.

\vcmnt{Creating an environment for the public where majority of them get vaccinated at ESSS and majority of the influencers get vaccinated is where the free riding behaviour is curbed. This turns out to be the least incentive scenario for the leader, and is feasible when  when the certainty level is too high and when the sensitivity of the public is very small. On the other hand, when relatively lower certainty level is desired, then the leader can induce an environment where very few influencers are vaccinated, and which is still sufficient for complete eradication, but this is possible when the sensitivity is too high. 

Surprisingly the leader has to work hard, when the public is dependent on influencers to a medium level and 
when the required level of certainty is high. 

For intermediate levels of sensitivity, the leader has to provide more incentives (work hard?)}

